A Multiobjective Approach for Sector Duration Optimization in Stereotactic Radiosurgery Treatment Planning

Sector duration optimization (SDO) is a problem arising in treatment planning for stereotactic radiosurgery on Gamma Knife. Given a set of isocenter locations, SDO aims to select collimator size configurations and irradiation times thereof such that target tissues receive prescribed doses in a reasonable amount of treatment time, while healthy tissues nearby are spared. We present a multiobjective linear programming model for SDO to generate a diverse collection of solutions so that clinicians can select the most appropriate treatment. We develop a generic two-phase solution strategy based on the epsilon-constraint method for solving multiobjective optimization models, which aims to systematically increase the number of high-quality solutions obtained, instead of conducting a traditional uniform search. To improve solution quality further and to accelerate the procedure, we incorporate some general and problem-specific enhancements. Moreover, we propose an alternative version of our two-phase strategy, which makes use of machine learning tools to reduce the computational effort. In our computational study on eight previously treated real test cases, a significant portion of obtained solutions outperformed clinical results and those from a single-objective model from the literature. In addition to significant benefits of the algorithmic enhancements, our experiments illustrate the usefulness of machine learning strategies to reduce the overall run times nearly by half while maintaining or besting the clinical practice.

==> Figures/fig_DVH.tex <==
\begin{figure}[H]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.5]{Figures/DVH_isoline/c6t1_DVH_RelativeDose_RegularRuns_NotDomAmongCov98PI75.pdf}
	\end{subfigure}
	~\hspace{0.9cm}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.5]{Figures/DVH_isoline/c6t1_DVH_AbsoluteDose_RegularRuns_NotDomAmongCov98PI75.pdf}
	\end{subfigure}
	\caption{Dose-volume histograms using relative dose percentages (left) and absolute doses (right) for Case 3. Relative dose percentages are computed with respect to the prescribed dose for the tumor, and maximum allowed doses for OARs. Solid and dashed gray vertical lines on the right correspond to the prescribed dose level for the tumor and maximum allowed dose for the two OARs, brainstem (BS) and cochlea, respectively...............}
	\label{fig:..........}
\end{figure}

==> Figures/fig_isodose.tex <==
\begin{figure}[H]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.5]{Figures/DVH_isoline/c6t1_ip300_largev_mar_20_LP_optBOT_isoPTVMar30_Tumor1_RegularRuns_R1_UBcombIndex92.png}
	\end{subfigure}
	~\hspace{0.9cm}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.5]{Figures/DVH_isoline/c6t1_ip300_largev_mar_20_LP_optBOT_isoPTVMar30_Tumor1_RegularRuns_R2_UBcombIndex5.png}
	\end{subfigure}
	\caption{Isodose lines of two selected treatment plans for Case 3. (BS: brainstem, Rx: prescribed dose for the tumor.)..............}
	\label{fig:..........}
\end{figure}

==> Figures/fig_notdomplots.tex <==
\section*{Only not-dominated results (wrt cov, PI, BOT)}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c3t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c3t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c3t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c3t1_BOT_PI}
	\end{subfigure}
	\caption{c3t1}
	\label{fig:c3t1}
\end{figure}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c3t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c4t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c4t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c4t1_BOT_PI}
	\end{subfigure}
	\caption{c4t1}
	\label{fig:c4t1}
\end{figure}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c6t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c6t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c6t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c6t1_BOT_PI}
	\end{subfigure}
	\caption{c6t1}
	\label{fig:c6t1}
\end{figure}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c7t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c7t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c7t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c7t1_BOT_PI}
	\end{subfigure}
	\caption{c7t1}
	\label{fig:c7t1}
\end{figure}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c11t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c6t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c11t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c11t1_BOT_PI}
	\end{subfigure}
	\caption{c11t1}
	\label{fig:c11t1}
\end{figure}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c12t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c12t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c12t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c12t1_BOT_PI}
	\end{subfigure}
	\caption{c12t1}
	\label{fig:c12t1}
\end{figure}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c13t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c13t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c13t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c13t1_BOT_PI}
	\end{subfigure}
	\caption{c13t1}
	\label{fig:c13t1}
\end{figure}

\begin{figure}[!h]
    \centering
	\begin{subfigure}{0.4\textwidth}
		\centering
	    \includegraphics[scale=0.55]{Figures/notDominated_cov_vs_PI/c14t1_5obj_BothPhases_Regular_ML_NotDom_Cov_vs_PI.pdf}
        % \caption{All data}
        %\label{subfig:c14t1_PI_cov}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\centering
        \includegraphics[scale=0.55]{Figures/notDominated_covThres997/c14t1_5obj_BothPhases_Regular_ML_CovThres997_NotDom_BOT_vs_PI.pdf}
        % \caption{Tumor coverage = 1}
        %\label{subfig:c14t1_BOT_PI}
	\end{subfigure}
	\caption{c14t1}
	\label{fig:c14t1}
\end{figure}



==> Models/model_5obj_dual.tex <==
\underline{\bf Dual: }
\begin{alignat*}{4}
&\text{max}& \qquad & - \ \sum_{\structure \in \setStructure} \sum_{\voxel \in \setVoxel_{\structure}}  \targetDose_{\structure}^{\max} \ \dualVarOverdoseCons_{\structure \voxel} 
\ - \ \sum_{\tumor \in \setTumor} \sum_{\voxel \in \setVoxel_{\tumor}}  \targetDose_{\tumor}^{\max} \dualVarOverdoseCons_{\tumor \voxel}
\ + \ \sum_{\tumor \in \setTumor} \sum_{\voxel \in \setVoxel_{\tumor}}  \targetDose_{\tumor} \ \dualVarUnderdoseCons_{\tumor \voxel}  
\ + \ \sum_{\objIndex=2}^{5} \dualVarEpsCons_{\objIndex} \ \eps_{\objIndex} 
\ - \ \sum_{\tumor \in \setTumor} \dualVarCovCons_{\tumor} \ \targetDose_{\tumor} \ |\setVoxel_{\tumor}| \ (1-\cov_{\tumor}) \\[0.25cm] %\label{obj5:dualobj}
%
&\text{s.t.}& \qquad & \dualVarObjCons_{\objIndex}  \ = \ 1 \qquad && \\[0.05cm]
%
&& \qquad & \dualVarObjCons_{\objIndex} \ + \ \dualVarEpsCons_{\objIndex} \ = \ 0 \qquad && \objIndex \in \{2, \ldots, 5\} \\[0.05cm]
%
%&\text{s.t.}& \qquad & \dualVarObjCons_{1} \ + \ \dualVarEpsCons_{1} \sum_{\objIndex = 2}^{\numObjs} \mathbbm{1}_{\{\objOrdering(\objIndex) = 1\}}  \ = \ \mathbbm{1}_{\{\objOrdering(1) = 1\}} \\[0.05cm]
%
%&& \qquad & \dualVarObjCons_{2} \ + \ \dualVarEpsCons_{2} \sum_{\objIndex = 2}^{\numObjs} \mathbbm{1}_{\{\objOrdering(\objIndex) = 2\}} \ = \ \mathbbm{1}_{\{\objOrdering(1) = 2\}} \\[0.05cm]
%
%&& \qquad & \dualVarObjCons_{3} \ + \ \dualVarEpsCons_{3} \sum_{\objIndex = 2}^{\numObjs} \mathbbm{1}_{\{\objOrdering(\objIndex) = 3\}} \ = \ \mathbbm{1}_{\{\objOrdering(1) = 3\}} \\[0.05cm]
%
%&& \qquad & \dualVarObjCons_{4} \ + \ \dualVarEpsCons_{4} \sum_{\objIndex = 2}^{\numObjs} \mathbbm{1}_{\{\objOrdering(\objIndex) = 4\}} \ = \ \mathbbm{1}_{\{\objOrdering(1) = 4\}} \\[0.05cm]
%
%&& \qquad & \dualVarObjCons_{5} \ + \ \dualVarEpsCons_{5} \sum_{\objIndex = 2}^{\numObjs} \mathbbm{1}_{\{\objOrdering(\objIndex) = 5\}} \ = \ \mathbbm{1}_{\{\objOrdering(1) = 5\}} \\[0.1cm]
%
&& \qquad & - \dualVarObjCons_{1} \ \sum_{\oar \in \setOAR} \sum_{\voxel \in \setVoxel_{\oar}}  \doseMat_{\oar \voxel \isocenter \sector \sectorSize}  
\ + \ \sum_{\tumor \in \setTumor} \sum_{\voxel \in \setVoxel_{\tumor}}  \doseMat_{\tumor \voxel \isocenter \sector \sectorSize} \ \dualVarUnderdoseCons_{\tumor \voxel} 
\ - \  \sum_{\structure \in \setRing \cup \setTumor} \sum_{\voxel \in \setVoxel_{\structure}}  \doseMat_{\structure \voxel \isocenter \sector \sectorSize} \ \dualVarOverdoseCons_{\structure \voxel} 
\ - \ \dualVarBOTCons_{\isocenter \sector} \ \leq \ 0 
\qquad &&  \isocenter \in \setIsocenter, \ \sector \in \setSector, \ \sectorSize \in \setSectorSize \\[0.15cm] % \label{obj5:dualcons1} 
%
&&\qquad &  -\dualVarObjCons_{2} \ + \ \dualVarOverdoseCons_{\ring \voxel}  \ \leq \ 0 &&\ring \in \setRing, \ \voxel \in \setVoxel_{\ring}  \\[0.05cm] %\label{obj5:dualcons2}
%
&&\qquad & -\dualVarObjCons_{3} \ + \  \dualVarOverdoseCons_{\tumor \voxel} \ \leq \ 0 &&\tumor \in \setTumor, \ \voxel \in \setVoxel_{\tumor}  \\[0.05cm] %\label{obj5:dualcons3}
%
&&\qquad & -\dualVarObjCons_{4} \ + \  \dualVarUnderdoseCons_{\tumor \voxel} \ - \  \dualVarCovCons_{\tumor} \ \leq \ 0 &&\tumor \in \setTumor, \ \voxel \in \setVoxel_{\tumor} \\[0.05cm] %\label{obj5:dualcons4} 
%
&&\qquad &  -\dualVarObjCons_{5} \ + \ \sum_{\sector \in \setSector} \dualVarBOTCons_{\isocenter \sector} \ \leq \ 0 &&\isocenter \in \setIsocenter  \\[0.05cm] %\label{obj5:dualcons5}
%
&&\qquad &  \dualVarEpsCons_{\objIndex} \  \leq \ -\dfrac{\epsilon}{\objRange_{\objIndex}} && \objIndex \in \{2, \ldots, 5\}  \\[0.05cm]  %\label{obj5:dualcons6}
%
&&\qquad & \dualVarOverdoseCons_{\structure \voxel} \ \geq \ 0 &&\structure \in \setStructure, \ \voxel \in \setVoxel_{\structure}  \\[0.05cm] 
%
&&\qquad &  \dualVarUnderdoseCons_{\tumor \voxel} \ \geq \ 0 &&\tumor \in \setTumor, \ \voxel \in \setVoxel_{\tumor} \\[0.05cm]
%
&&\qquad &  \dualVarBOTCons_{\isocenter \sector} \ \geq \ 0 && \isocenter \in \setIsocenter, \ \sector \in \setSector  \\[0.05cm]
%
&&\qquad &  \dualVarCovCons_{\tumor} \ \geq \ 0 && \tumor \in \setTumor 
%&&\qquad &  -\dualVarEpsCons_{\objOrdering(1)} \ \leq \ 0  && %\label{obj5:dualcons7}
\end{alignat*} 


==> PseudoCodes/algo_2phase.tex <==
% OUR MULTI-PHASE SOLUTION APPROACH AND PSEUDO-CODES WILL COME SOMEWHERE HERE (FIRST PASS FOR DETERMINING PROMISING REGIONS, THE REST FOR TAKING RUNS IN THE CONFINED RANGES)

% WHAT I DID CURRENTLY: AFTER THE SECOND ROUND, I DECREASED THE UB OF BOT TO VALUES THAT ARE NOT TOO MUCH ABOVE THE CLINICAL ONES. ALSO. EVEN THOUGH THE FILTERINGS INCREASE THE LB ON TUMOR UNDERDOSE, I KEPT THEM AS IS IN ORDER NOT TO DETERIORATE THE COVERAGE VALUES POTENTIALLY

{
\color{blue}
THE FOLLOWING ALGORITHM MAY BE REVISED LATER ON...
}

{
\newcommand{\model}{\mathcal{M}}
\newcommand{\phaseIter}{k}
\newcommand{\clinResults}{C}
\newcommand{\sdoInstance}{I}

\begin{algorithm}
\vspace*{0.15cm}
    \caption{Two-phase approach...}\label{algo:2phase} 
    \hspace*{\algorithmicindent}{\bf Input:} An $\varepsilon$-constraint model $\model$ for an instance $\sdoInstance$ to the {\sdo} problem, clinical results $\clinResults$ for $\sdoInstance$\\
    \hspace*{\algorithmicindent}{\bf Output:} A set $\setPareto$ of Pareto-optimal points
    \begin{algorithmic}[1]
        \Procedure{Run}{}
            \State $ \setPareto \gets \varnothing $ %\Comment{Initialize set of nonbinding constraints}
            \ForAll{$ \phaseIter \in \{1,2\} $}
            \State $\epsSet \gets \varnothing $ 
            \If{ $\phaseIter = 1$ }
                \State Run Algorithm \ref{algo:grid} to set $\epsSet$ of grid points, using 20 grid points in the range of each objective %function $\objIndex \in \{1, \ldots, \numObjs\}$
            \Else
                \State Filter out the elements of $\setPareto$ whose coverage, PI, and BOT values are inferior to those in $\clinResults$ 
                \State Set the objective ranges using the minimum and maximum values of remaining points in $\setPareto$
                \State Set $\epsSet$ of grid points, using 10 grid points in the range of each objective function % $\objIndex \in \{1, \ldots, \numObjs\}$
            \EndIf
            \ForAll{$ \eps \in \epsSet $} %\Comment{Find the set of nonbinding constraints}
                \State Optimally solve $\model$ using $\eps$ 
                \If{ feasible } 
                    \State Let $\objVal_{\objIndex}$ for $\objIndex \in \{1, \ldots, \numObjs\}$ be the optimal objective values
                    \State $\setPareto \gets \setPareto \cup \{\objVal_1, \ldots, \objVal_{\numObjs}\} $ 
                    \State Run Algorithm \ref{algo:equiv} to discard the grid points which would give the same solution
                \Else
                    \State Run Algorithm \ref{algo:infeas} to discard the grid points whose infeasibility is implied
               \EndIf
            \EndFor
            \EndFor
        \EndProcedure
    \end{algorithmic}
\end{algorithm}
}

==> PseudoCodes/algo_detect_equiv.tex <==
{
\newcommand{\givenObjVal}{\objVarOptVal^{\prime}}
\newcommand{\givenObjUB}{\eps^{\prime}}

\begin{algorithm}
\vspace*{0.15cm}
    \caption{Early detection of repeating solutions}\label{algo:equiv} 
    {\bf Input:} An upper bound vector $\eps^{\prime}$, 
    some $\objVarOptVal^{\prime} \in \optObjSet(\eps^{\prime})$,
    and a set $\epsSet$ of $\eps$-vectors to check \\
    {\bf Output:} A subset $\epsSet^{\prime} \subseteq \epsSet$ excluding the $\eps$-vectors that can yield $\objVarOptVal^{\prime}$ as a vector of optimal objective values
    \begin{algorithmic}[1]
        \Procedure{DetectRepeating}{} \label{proc:detect_equiv}
            % \State  \Comment{Initialize set of nonbinding constraint indices}
            \State $ \nonbindingSubset \gets \varnothing, \ \epsSet^{\prime} \gets \epsSet$
            \ForAll{$ \objIndex \in \{2, \ldots, \numObjs\}$} %\Comment{Find the set of nonbinding constraints}
                \If{ $ \givenObjVal_{\objIndex} < \givenObjUB_{\objIndex} $ } 
                % \State 
                $ \nonbindingSubset \gets \nonbindingSubset \cup \{\objIndex \} $
                \EndIf
            \EndFor
            \If{ $ \nonbindingSubset \neq \varnothing $} %\Comment{If there are nonbinding constraints}
                \ForAll{$\eps \in \epsSet$} %\Comment{Check equivalence of combinations}
                    \If{$ \givenObjVal_{\objIndex} \leq \eps_{\objIndex} \ \ \forall \objIndex \in \nonbindingSubset \algoand \eps_{\bindingSubsetIndex} = \givenObjUB_{k} \ \ \forall \bindingSubsetIndex \in \{2, \ldots, \numObjs\} \setminus \nonbindingSubset  $ }
                    % \State 
                    $ \epsSet^{\prime} \gets \epsSet^{\prime} \setminus \{\eps\}$
                    \EndIf
                \EndFor
            \EndIf
        \EndProcedure
    \end{algorithmic}
\end{algorithm}
}

==> PseudoCodes/algo_detect_infeas.tex <==
{
\newcommand{\givenEps}{\eps^{\text{infeas}}}

\begin{algorithm}
\vspace*{0.15cm}
    \caption{Early detection of infeasibilities}\label{algo:infeas} 
    {\bf Input:} An upper bound vector $\givenEps$
    leading to infeasibility, and a set $ \epsSet $ of upper bound vectors to check \\
    {\bf Output:} A subset $\epsSet^{\prime} \subseteq \epsSet$ that does not contain $\eps$-vectors for which infeasibility is implied by $\givenEps$
    \begin{algorithmic}[1]
        \Procedure{DetectInfeasible}{}
            \State $\epsSet^{\prime} \gets \epsSet$
            \ForAll{$\eps \in \epsSet$} 
            \If{ $\eps_{\objIndex} \leq \givenEps_{\objIndex} \ \ \forall \objIndex \in \{2, \ldots, \numObjs\} $} 
            % \State 
            $ \epsSet^{\prime} \gets \epsSet^{\prime} \setminus \{\eps \} $
            \EndIf
            \EndFor
        \EndProcedure
    \end{algorithmic}
\end{algorithm}
}

==> PseudoCodes/algo_predict_feas.tex <==
\begin{algorithm}
\vspace*{0.15cm}
    \caption{\cred Predict and find promising upper bound vectors}
    \label{algo:predictselect}  
    {\bf Input:} A training set $\left\{\left(\coverage(\allVars), \PI(\allVars), \BOTVal(\allVars) \right) \colon \allVars = \optSol \text{~for some~} \optSol \in \optSolSet(\eps), \eps \in \epsSetTrain \right\}$ with $\epsSetTrain$ a set of upper bound vectors, a set $\epsSet$ to make predictions for, and threshold values $\coverageThres$, $\PIThres$, $\BOTThres$ \\
    {\bf Output:} A set $\epsSet^{\prime}$ of selected upper bound combinations %whose predicted $\left\{\left(\coverage(\eps), \PI(\eps), \BOTVal(\eps) \right)\right\}_{\eps \in \epsSet^{\prime}}$ is not dominated among others
    \begin{algorithmic}[1]
        \Procedure{PredictPerformanceAndSelect}{}
        \State $\predFnc_{\coverage}(.) \gets \trainFnc_{\coverage} 
        \left( \left\{ \big( \eps, \coverage(\allVars) \big) \colon \allVars = \optSol \text{~for some~} \optSol \in \optSolSet(\eps), \eps \in \epsSetTrain \right\} \right)$ 
        \State $\predFnc_{\PI}(.) \gets \trainFnc_{\PI} 
        \left( \left\{ \big( \eps, \PI(\allVars) \big) \colon \allVars = \optSol \text{~for some~} \optSol \in \optSolSet(\eps), \eps \in \epsSetTrain \right\} \right)$ 
        \State $\predFnc_{\BOTVal}(.) \gets \trainFnc_{\BOTVal} 
        \left( \left\{ \big( \eps, \BOTVal(\allVars) \big) \colon \allVars = \optSol \text{~for some~} \optSol \in \optSolSet(\eps), \eps \in \epsSetTrain \right\} \right)$ 
        \State $\epsSet^{\prime} \gets \varnothing$
        \ForAll {$\eps \in \epsSet$}
            % \State $(\coverage^{\text{pred}}, \PI^{\text{pred}}, \BOTVal^{\text{pred}}) \gets \predFnc(\eps)$
            \State $\coverage^{\text{pred}} \gets \predFnc_{\coverage}(\eps), \ \PI^{\text{pred}} \gets \predFnc_{\PI}(\eps), \ \BOTVal^{\text{pred}} \gets \predFnc_{\BOTVal}(\eps)$
            \If{$\PI^{\text{pred}} \geq \PIThres \algoand \coverage^{\text{pred}} \geq \coverageThres \algoand \BOTVal^{\text{pred}} \leq \BOTThres \ $}
            \State $\ \epsSet^{\prime} \gets \epsSet^{\prime} \cup \{\eps\}$
            \EndIf
        \EndFor
        \EndProcedure
    \end{algorithmic}
\end{algorithm}



==> PseudoCodes/algo_set_grids.tex <==

{
\newcommand{\givenObjUB}{\eps^{\prime}}
\newcommand{\givenObjUBSet}{\epsSet}
\newcommand{\gridIter}{j}
\newcommand{\increment}{\Delta}

\begin{algorithm}
\small
\vspace*{0.15cm}
    \caption{Setting the $\eps$-vectors}\label{algo:grid}  
    {\bf Input:} Number of equidistant points $ \numGrids_{\objIndex} \geq 2 $ on the range of objective $\objVar_{\objIndex}$ for $\objIndex \in \{2, \ldots, \numObjs\}$ \\
    {\bf Output:} The sets $\epsSet_{\objIndex}$ of $\eps_{\objIndex}$'s for $\objIndex \in \{2, \ldots, \numObjs\}$ and the set $\epsSet$ of all $\eps$-vectors
    \begin{algorithmic}[1]
        \Procedure{Set$\eps$-Vectors}{}
        \ForAll {$\objIndex \in \{2, \ldots, \numObjs\}$} 
            \State $ \eps_{\objIndex}^1 \gets \objRangeLB_{\objIndex}, \ \epsSet_{\objIndex} \gets \{\eps_{\objIndex}^1\}, \  \increment_{\objIndex} \gets \frac{\objRangeUB_{\objIndex}-\objRangeLB_{\objIndex}}{\numGrids_{\objIndex} - 1}$
            \ForAll { $ \gridIter \in \{2, \ldots, \numGrids_{\objIndex}\} $ }
                \State $ \eps_{\objIndex}^{\gridIter} \gets  \eps_{\objIndex}^{\gridIter-1} + \increment_{\objIndex} $, \  $\epsSet_{\objIndex} \gets \epsSet_{\objIndex} \cup \{ \eps_{\objIndex}^{\gridIter} \}$
            \EndFor
        \EndFor
        \State $ \epsSet \gets \epsSet_{2} \times \ldots \times \epsSet_{\numObjs} $
        \EndProcedure
    \end{algorithmic}
\end{algorithm}
}



==> Tables/table_payoff.tex <==
\begin{table}[!h]
\centering
	\caption{A payoff table for a multiobjective problem with $\numObjs$ objectives.}
	\label{tab:payoff}
	\scalebox{0.9}{
    \begin{tabular}{M{1.3cm}M{0.8cm}M{0.8cm}M{0.8cm}M{0.8cm}M{0.8cm}}
    	\toprule
    	& \multicolumn{1}{c}{ $\boldsymbol{\objVar_1}$} & \multicolumn{1}{c}{ $\boldsymbol{\ldots}$} & \multicolumn{1}{c}{ $\boldsymbol{\objVar_\payoffIndex}$} & \multicolumn{1}{c}{ $\boldsymbol{\ldots}$} & \multicolumn{1}{c}{ $\boldsymbol{\objVar_{\numObjs}}$}  \\
    	\midrule
    	{ $\boldsymbol{\payoffModel_1}$ } & $\objVal_{1}^{1}$ & \multicolumn{1}{c}{$\ldots$} & $\objVal_{\payoffIndex}^{1}$ & \multicolumn{1}{c}{$\ldots$} & $\objVal_{\numObjs}^{1}$\\[0.05cm]
    	%
    	\multicolumn{1}{c}{$\boldsymbol{\vdots}$} &\multicolumn{1}{c}{$\vdots$} & \multicolumn{1}{c}{$\ddots$} & \multicolumn{1}{c}{$\vdots$} & \multicolumn{1}{c}{$\ddots$} & \multicolumn{1}{c}{$\vdots$}\\[0.05cm]
    	%
        { $\boldsymbol{\payoffModel_{\payoffIndex}}$ } & $\objVal_{1}^{\payoffIndex}$ & \multicolumn{1}{c}{$\ldots$} & $\objVal_{\payoffIndex}^{\payoffIndex}$ & \multicolumn{1}{c}{$\ldots$} & $\objVal_{\numObjs}^{\payoffIndex}$\\[0.05cm]
        %
    	\multicolumn{1}{c}{$\boldsymbol{\vdots}$} &\multicolumn{1}{c}{$\vdots$} & \multicolumn{1}{c}{$\ddots$} & \multicolumn{1}{c}{$\vdots$} & \multicolumn{1}{c}{$\ddots$} & \multicolumn{1}{c}{$\vdots$}\\[0.05cm]
    	%
    	{ $\boldsymbol{\payoffModel_{\numObjs}}$ } & $\objVal_{1}^{\numObjs}$ & \multicolumn{1}{c}{$\ldots$} & $\objVal_{\payoffIndex}^{\numObjs}$ & \multicolumn{1}{c}{$\ldots$} & $\objVal_{\numObjs}^{\numObjs}$ \\[0.05cm]
    	\bottomrule
    \end{tabular}%
    }
\end{table} 


==> introduction.tex <==
\section{Introduction}

%brief info about radiotherapy
Radiotherapy is one of the most commonly used cancer treatment methods.
The technique uses high-energy radiation to kill or damage cancer cells,
% {\crevi , which uses high-energy radiation to kill or damage cancer cells.}
and is employed in approximately half of the treatments, sometimes in conjunction with chemotherapy and surgery~\citep{breedveld2019multi}.
%\st{Radiotherapy uses high-energy radiation to kill or damage cancer cells. During the delivery of radiation beams to tumors, normal tissues may inevitably be damaged as well, even with the state-of-the-art equipment and techniques. Therefore, the goal in radiotherapy is to administer prescribed doses of radiation to tumors with least possible exposure of healthy tissues nearby.}
%then radiosurgery
There are different forms of radiotherapy, one of which is {\it stereotactic radiosurgery} ({\srs}), {\crevi a technique specifically designed to deliver high doses of radiation from multiple positions to precisely defined targets in the brain.} 
% using narrow beams of radiation delivered from multiple positions meeting at a single target with submillimeter accuracy.}
%\st{Developed originally by neurosurgeon Lars Leksell \citep{leksell1951stereotactic}, {\srs} involves using multiple narrow beams of radiation arranged on a three dimensional reference system, which meet at a single target with submillimeter accuracy.} 
%\st{Whereas conventional radiotherapy techniques give small doses repeatedly over a period of time, {\srs} delivers high (``surgical") doses in a single session by means of a spatially distributed approach, typically to small tumors \citep{webb1993physics,chen2005stereotactic}. Since the dose delivered to a single point is high, precise targeting is particularly crucial in this method. Due to the distributed delivery from multiple positions, the beams exert little effect on the structures they pass through, yet the desired dose is attained at the target where the beams converge. In this way, {\srs} can better spare the tissues surrounding the targets from any significant dose.}
%\st{Over the last several decades, various types of {\srs} delivery systems have been developed, which differ in the radiation source used and the way beams are concentrated at the target.}
{\gk} was the first {\srs} delivery system, but the state of the art is Leksell Gamma Knife\textsuperscript{\textregistered} ({\lgk}) Icon{\texttrademark} by Elekta (Stockholm, Sweden)~\citep{zeverino2017}.
%\st{{\lgkicon} is different from the former models mainly by the design of its beam delivery and patient positioning systems as well as planning software \citep{lindquist2007leksell,zeverino2017}.}
% \st{, through which a high level of automation and flexibility is provided \citep{lindquist2007leksell,zeverino2017}. }

{\lgkicon} (and also its predecessor {\perfexion}) has eight independently controlled {\it sectors} and contains 192 cobalt-60 (a radioactive isotope) sources, 24 per sector.
Each sector can be robotically moved to one of the three circular {\it collimator sizes} (with 4, 8, and 16 mm diameters) or be blocked. 
All the sources in a sector deliver radiation beams through the chosen size, or are completely blocked. 
A patient lies still on a treatment couch and radiation beams are emitted from the sectors to the target, where their focal point is termed an {\it isocenter}.
The couch remains stationary while radiation is being delivered to a specific isocenter and is repositioned automatically for other isocenter locations defined in the treatment plan. 
{\crevii All beams are blocked as the patient is repositioned.}
Each isocenter is irradiated for a certain amount of time through one or more collimator configurations, and the treatment session
%is completed once the target sites are delivered the planned radiation amounts.
{\crevii is complete once the planned radiation amounts have been delivered to each isocenter.}

{\crevi 
Different types of radiotherapy techniques require similar decisions to be made to determine a treatment plan. 
{\crevii Common decisions include the irradiation times as well as the positions and aperture shapes and/or sizes through which radiation beams target cancerous regions.}
% to send the beams from and the radiation amount through each selection, which need to be adapted to the specifics of the delivery device. 
For {\gk} systems, a set of aperture sizes at every sector is fixed on the device, and the planner needs to decide on the irradiation durations for each of~them.
%For instance, a widely-used equipment in linear accelerator-based delivery systems is multileaf collimators (MLCs), which consist of pairs of parallel metal leaves that can move horizontally and thereby shape the aperture radiation beams pass through \citep{srsbook2019ch7}. For these systems, %which are commonly used in intensity modulated radiation therapy (IMRT), 
%it is necessary to decide on the radiation amount to deliver, as well as the configuration(s) of MLC leaves at all possible beam directions along the arc(s) the device rotates on. For {\gk} systems, on the other hand, a set of aperture sizes at every sector are fixed on the device, and the planner needs to decide on the irradiation durations for each of~them.
}

{\srs} treatment planning %\st{with {\lgkicon}} 
% can be considered to be comprised of two main steps: 
has two main steps, those being 
(i) determination of the number and locations of isocenters, and (ii) finding the irradiation times of each isocenter. 
Existing studies mostly {\crevii handle} %\st{deal with}
these two problems separately.
For the former, heuristic methods are commonly used; for instance, \cite{ghobadi2012automated} combine the well-known grassfire algorithm \citep{wagner2000geometrically} with sphere packing, and \cite{doudareva2015skeletonization} introduce a method based on skeletonization techniques.
We focus on the latter problem in this study.
% In this study, we focus on the latter problem, which we describe next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Problem Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given a set of isocenter locations, {\crevii the} {\it sector duration optimization} ({\sdo}) problem {\crevii aims to find} the irradiation durations of every isocenter from each sector through each collimator size, such that a quality solution is achieved in terms of {\crevi clinical goals}. % \st{clinical goals of the treatment plan. }
%why it is challenging
{\crevi The problem %\st{is challenging because it} 
has high dimensionality and incorporates a large number of clinical restrictions.} 
%\st{incorporates a large number of clinical restrictions. Dose and avoidance limitations need to be satisfied for each unit volume of the target and surrounding structures, which translates into an extensive set of constraints.}
Consequently, it is not generally possible to generate an optimal {\crevi or clinically acceptable} treatment plan simply by inspection, 
%\st{while even suboptimal but clinically acceptable plans are difficult to develop. Thus, } 
thus mathematical models and optimization tools are needed. 


%multiobjective modeling motivations go here
{\crevi As in other radiotherapy problems, multiple criteria are considered in {\sdo}. Target sites should receive the prescribed doses, while surrounding tissues should be spared.}
%\st{First, target sites need to receive the prescribed doses. While delivering radiation to the targets, however, normal healthy tissues may inevitably be exposed to some dose. Therefore, keeping the irradiation of surrounding tissues at a minimal level emerges as another goal of {\sdo}.}
The duration of the treatment is another important consideration, because longer treatment times may cause patient discomfort and increases the possibility of patient movement leading to dose uncertainties \citep{srsbook2019ch7}.
These and other criteria are {\crevi commonly considered in radiotherapy treatment planning. They are} conflicting in nature, and it is generally not possible to simultaneously attain individual best values for each. 
%Deciding on the goodness of a treatment plan through a single objective value {\crevi may cause} %\st{causes} one to overlook alternative plans that cannot be deemed superior to one another on the basis of a vector of objective values.
{\crevi Moreover,} clinicians are often interested in evaluating trade-offs among competing criteria %{\crevi on the basis of a set of criteria} 
and choosing a plan most suitable to the specifics of a case.
%{\crevi Our multiobjective approach yields a collection of plans and serves this purpose well.}
{\crevii Motivated by this,}
%, which we propose in this study.}
%\st{This necessitates a multiobjective approach yielding a collection of plans, which we propose in this study.}
\begin{comment}
%why it is not good to use a single-objective for a problem with inherently multiple objectives
For problems involving multiple objectives, %\st{the notion of simultaneous minimization (or maximization) is not well-defined.}
%\st{deterioration in one objective may lead to an improvement in another, and such changes do not necessarily impose a dominance relation among different solutions.}
%\st{As {\sdo} naturally incorporates multiple goals, }
deciding on the goodness of a treatment plan through a single objective value {\crevi may cause} %\st{causes} 
one to overlook alternative plans that cannot be deemed superior to one another on the basis of a vector of objective values.
%\st{A single-objective model produces one optimal solution, unless alternative optima exist and are explicitly sought. However,} 
{\crevi Also,} clinicians are often interested in evaluating different trade-offs and choosing a plan most suitable according to the specifics of each case.
This necessitates a multiobjective approach yielding a collection of plans, which we propose in this study.
\end{comment}
%\subsection{Our Work}
%\st{In this study,} 
we {\crevii propose} a multiobjective approach for {\sdo} arising in {\srs} treatment planning {\crevi on Gamma Knife systems}, particularly with {\lgkicon}.
Our aim is to provide a collection of solutions addressing the trade-offs between conflicting clinical goals, and thereby offer flexibility to decision makers {\crevii as they select a plan for an individual patient.}
% to opt for treatment plans depending on patient-specific needs.
%\st{To the best of our knowledge, this is the first study adopting such a multiobjective approach for {\sdo} with this particular generation of {\gk} devices.}

{\crevi We present a multiobjective linear programming model for {\sdo}, %\st{with five objectives}, 
with the the objectives being to minimize the underdosing of tumors, the overdosing of tumors and healthy tissues, and the treatment time.}
%NOTE FROM OYLUM: WHY DOES HE SAY THREE OBJECTIVES?????????????????
%\st{and} 
We introduce a two-phase solution approach that employs {\crevii a widely-used technique}
% an existing method 
to solve multiobjective optimization models, namely, the $\eps$-constraint method,
{\crevi which consists of optimizing one objective while bounding the others.}
% {\crevii  We introduce a two-phase solution approach that employs a widely-used technique to solve general multiobjective optimization models, namely, the $\eps$-constraint method, and is capable of generating all Pareto-optimal points in theory by varying the bounds.}
We perform the first phase to explore solutions from all parts of the feasible space, and the second phase to restrict the search to achieve a denser representation of clinically desirable solutions. 
{\crevi Generated solutions yield Pareto-optimal points in terms of the model objectives; however, we continue the evaluative process by evaluating a treatment plan with some widely-used clinical measures, namely, tumor coverage and Paddick conformity index. Note that these clinical metrics are not directly optimized by the model, and 
in that regard, our objectives, other than the treatment time, serve as surrogates to derive solutions that yield clinically preferable options.}
%\st{To test the performance of our approach, }
We conduct computational experiments using anonymized data from eight previously treated cases, and we compare our results with the clinical plans and the treatment plans from the single-objective model by \cite{cevik2019simultaneous}.
{\crevi
% ,  and thereby illustrate the performance of our strategies in generating a diverse set of high-quality treatment plans.
We note that even though we demonstrate our solution scheme on the SDO problem with {\lgkicon}, it is a generic framework that can be applied to other radiosurgery modalities, and even other multiobjective problems.
}
% We generate a diverse collection of {\cred Pareto-optimal} points, which offers flexibility to decision makers to address the clinical trade-offs according to the unique and individual needs of each patient. 


%\subsubsection*{Contributions.}
Our main contributions {\crevii can be summarized as follows}:
% Our main contributions can be summarized as follows:
\begin{itemize}
    \item We present a multiobjective linear programming model for {\sdo} %\st{with {\lgkicon}} 
    and generate a diverse collection of solutions, offering flexibility to decision makers to select one that best suits patient-specific needs.
    We also derive inequalities that improve our model and that aid the solution process.
    % procedure to obtain clinically desirable solutions.  
    %
    \item We provide a self-contained alternative proof showing that a properly constructed $\eps$-constraint model yields an efficient solution for the multiobjective model.
    %
    \item We prevent generation of repeating solutions in the $\eps$-constraint method by extending an existing strategy to linear programs, applicable regardless of problem context. 
    %
    \item We propose a generic and efficacious two-phase $\eps$-constraint method, {\twophase}, that systematically focuses the search on more favorable regions. We additionally develop an alternative version of {\twophase} that makes use of machine learning tools to predict performance, which thereby reduces the computational burden.
   % \item \st{We conduct a detailed numerical study using clinical instances, illustrating the performance of our approaches in generating a diverse set of high-quality treatment plans.}
\end{itemize}


%\subsubsection*{Paper organization.}
{\crevi
{\crevii The rest of the paper is organized as follows.} We survey the related literature in Section~\ref{sec:literature} and present our multiobjective model for SDO in Section~\ref{sec:model}.
We then review the $\varepsilon$-constraint method and propose problem-specific improvements in Section~\ref{sec:epscons}, and we provide algorithmic enhancements in Section~\ref{sec:enhancements}.
We introduce {\twophase} in Section~\ref{sec:twophase}, report our experimental results in Section~\ref{sec:expresults}, and conclude our work in Section~\ref{sec:conc}.
%finally give a brief summary and future research directions in Section \ref{sec:conc}.
We provide all the proofs in the Online Supplement.
}

\begin{comment}
\st{
\subsection{Paper Organization}
The rest of this paper is organized as follows. 
In Section~\ref{sec:model}, we present our multiobjective linear programming model for SDO.
In Section~\ref{sec:epscons}, we review the $\varepsilon$-constraint method and propose various novel problem-specific improvements.
We then present algorithmic enhancements to the $\varepsilon$-constraint method in Section~\ref{sec:enhancements}, which significantly accelerate the solution procedure.
In Section~\ref{sec:twophase}, we introduce our two-phase $\eps$-constraint method with two alternative versions, and follow it with the results of our experimental study conducted on real clinical cases in Section~\ref{sec:expresults}.
Finally, we conclude our study in Section~\ref{sec:conc} with a brief summary and future research directions.
We provide all the proofs in the Online Supplement.
}
\end{comment}




==> outline.tex <==
\section*{Outline}
TENTATIVE OUTLINE OF THE PAPER
\begin{itemize}
    \item Introduction
    \begin{itemize}
        \item Define the problem
        \item Why it is important, relevance
        \item Emphasize that it has conflicting objectives by its nature
        \item Related literature on the topic
    \end{itemize}
    \item The model
    \begin{itemize}
        \item Give the main constraints of the model
        \item Discuss the objectives of this problem in more concrete terms
        \item Say that we are going to make this a multiobjective model
        \item Introduce the objectives and discuss the motivation behind selecting them as such
        \item Give the models 
        \item Justify our need to use the dual models and give the duals
    \end{itemize}
    \item Solution method
    \begin{itemize}
        \item Give brief info about the eps constraint method
        \item Give some further info about Mavrotas' method
        \item Do we need to justify why this MOP method is selected and used, rather than others?
        \item The way we set the ranges for objective functions
        \begin{itemize}
            \item First, the payoff table discussion
            \item Then, narrowing down the ranges obtained
        \end{itemize}
        \item The way we generate Pareto opt solutions via grid points
        \item Our findings to discard identical solutions
        \item Some stats about how many grid point combos could be avoided with this approach
    \end{itemize}
    \item Experimental results
    \begin{itemize}
        \item Info about the instances; that they are real and they are spectacular :)
        \item Info about instance sizes
        \item That we have used clinical coverage values as the minimum desired coverage values
        \item Chart: x-axis: instances, y-axis: Coverage values. One line for clinical coverage values, and one line for the coverage values of our model output
        \item Tables for detailed results
    \end{itemize}
    \item Discussion
    \begin{itemize}
        \item That it can be tried to incorporate actual clinical performance measures directly into the model
        \item That PI could be used to derive bounds for the ranges of objective fncs
    \end{itemize}
\end{itemize}


==> results.tex <==
\section{Experimental Results}
\label{sec:expresults}

%\st{In this section, we present the results of our computational study.}
We conducted our experiments on a MacOS computer with a 3 GHz Intel Core i5 CPU and 16 GB memory.
We used CPLEX 12.10 \citep{cplex1210} as linear programming solver,
and \texttt{scikit-learn} Python library \citep{scikit-learn} for our ML-related implementations.
%\st{We used the dual of the $\eps$-constraint formulation of our MOLP in \eqref{model:5obj}, because we observed significant run time reductions in our preliminary experiments, which is largely due to the sparsity of constraints in the dual model. }
%{\crevi We solved the dual of the $\eps$-constraint formulation of our MOLP using the primal simplex method, as our preliminary tests showed that it was the fastest option considering the combination of primal and dual formulations with all the applicable algorithms offered by CPLEX. Sifting algorithm was  approximately as fast for solving the dual, but was the slowest option in solving the primal. The barrier algorithm was slow both for the primal and dual, taking six to nine times more than the fastest option for either model. These choices significantly impact the total run times as we solve them a number of times.}

{\crevii 
% In order to decide on the fastest option, 
We considered combinations of the primal and dual formulations of the $\eps$-constraint formulation of our MOLP with all the applicable algorithms offered by CPLEX (including the ``automatic" option where the solver decides which algorithm(s) to use) to determine the fastest option. 
The average solution times of 77 $\varepsilon$-constraint models of a representative instance (Case 3) are provided in Table~\ref{tab:lp_algos}, which shows that solving the dual model with the primal simplex and sifting algorithms give the best overall performance. 
Since the two average times are quite close, we further compared the two options on another instance (Case 6) via 71 $\varepsilon$-constraint models. 
The average times were 4.53 and 5.67 seconds for primal simplex and sifting algorithms, respectively. 
Hence, we conducted our computational experiments by solving the dual formulation using the primal simplex method. }

\setlength{\tabcolsep}{9pt} % adjust column separation in table
\renewcommand{\arraystretch}{1.01} % adjust row separation in table
\begin{table}[!ht]
\crevii
    \centering
    \caption{\crevii Average solution times (in seconds).}
    \label{tab:lp_algos}%
    \resizebox{0.47\textwidth}{!}{
    \begin{tabular}{lrr}
    \toprule
    Algorithm & Primal model & Dual model\\
    \midrule
	Automatic &  10.16 &  7.74\\
	Primal simplex &  7.00 &  2.36\\
	Dual simplex &  3.91 &  4.96\\
	Barrier	&  27.89 &  21.08\\
	Concurrent	&  10.74 &  8.20\\
	Sifting	&  49.96 &  2.13\\
    \bottomrule
    \end{tabular}
    }
\end{table}

% \begin{table}[htbp]
% \crevii
%   \centering
%   \caption{Average solution times (in seconds).} %for different algorithms in solving the primal and dual formulations
%       \scalebox{0.71}{
%     \begin{tabular}{l S[table-format=1.2] S[table-format=1.2]}
% 	\toprule
%         \multicolumn{1}{l}{\parbox{3cm}{ Algorithm}} 	& \multicolumn{1}{c}{\parbox{3cm}{\centering Primal model}} 	& \multicolumn{1}{c}{\parbox{3cm}{\centering Dual model}} 	\\
% 	\midrule
%     	Automatic 						&  10.16 					&  7.74 		\\
%     	Primal simplex  					&  7.00      				&  2.36 		\\
%     	Dual simplex 						&  3.91   					&  4.96 	 	\\
%     	Barrier 							&  27.89     				&  21.08 		\\
%     	Concurrent 						&  10.74 					&  8.20  		\\
%     	Sifting 							&  49.96       				&  2.13 		\\
% 	\bottomrule
%     \end{tabular}%
%     }
%   \label{tab:lp_algos}%
% \end{table}%

We begin our empirical analysis by providing descriptive information on our test bed in Section~\ref{subsec:expresults_instinfo}.
Afterwards, we present summary statistics on the performance of {\twophase} in Section~\ref{subsec:expresults_2phase}, including the impact of the early detection strategies. 
Lastly, in Section~\ref{subsec:expresults_comparison}, we evaluate the solution quality of {\twophase}, and compare it to that of the single-objective linear program ({\cevikModel}) of \cite{cevik2019simultaneous}, and the actual clinical results obtained by applying the plans generated via the planning module Leksell GammaPlan\textsuperscript{\textregistered} \citep{leksellGammaPlan2010}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Test Bed}
\label{subsec:expresults_instinfo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our test instances consist of anonymized data of eight previously treated clinical cases with a single tumor, which are also used {\crevii by} \cite{cevik2019simultaneous}.
% We summarize some descriptive information about the instances in Table~\ref{tab:inst_info}. %, 
Table~\ref{tab:inst_info} lists descriptive information about the instances.
%{\cblue  namely the number of isocenters used (\# isocenters), prescribed dose for the tumor (Tumor prescr dose), maximum allowed doses for OARs (OAR dose limit), volume of the tumor (Tumor vol), number of voxels in the tumor, ring, and OARs (\# tumor/ring/OAR voxels), and total number of voxels (Total \# voxels). }

% including the number of isocenters used for each.
% , prescribed and maximum allowed doses for tumor and OARs (if any), as well as tumor volumes and the number of voxels in tumor, ring, and OARs  

\input{Tables/table_instance_info}
%
Isocenter locations are typically determined manually by the planners so that the overall tumor volume is adequately covered.
In theory, it is possible to use each tumor voxel as an isocenter, but the size of the model then grows prohibitively large and cannot be handled in practice.
% but their number being in the order of thousands, the size of the model as well as the input parameters, specifically the dose matrix $\doseMat$, would grow prohibitively large and cannot be handled in practice. 
Isocenters in our cases are positioned automatically with the grassfire and sphere packing algorithms~\citep{cevik2019simultaneous}.
% The ones in our test instances are set as explained in \citep{cevik2019simultaneous}, namely by using grassfire and sphere packing algorithms. 
We note that the quality of the generated treatment plans is quite robust to the number of isocenters, and potential effect of fewer isocenters is usually compensated for by the use of larger collimator sizes in delivering radiation, see for instance \citep{cevik2019simultaneous}.


% From Mucahit's SDIO paper
% In the clinical plans, isocenter locations are usually manually selected to span the tumor volume. Ideally any coordinate within the tumor volume can be a candidate for an isocenter location. However, even when we only take the tumor voxels to be candidate isocenter locations, we may end up with thousands of eligible isocenters, which would lead to computationally intractable SDIO models. As such, also to promote the automation in treatment plan generation, we use grassfire and sphere packing algorithms (GSP) to determine the eligible set of isocenters ( I ). If GSP generates a low number of isocenters, we use random sampling to increase the number of isocenters to 50 or 100 (depending on the experiment and instance).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Efficacy of Our Approach}
\label{subsec:expresults_2phase}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We first demonstrate the the efficacy of {\twophase}.
% Our goal in this section is to demonstrate the efficacy of {\twophase}. % together with the early detection procedures.
%Specifically, we show that infeasibilities and repeating solutions are prevalent, and the filters to avoid them give substantial benefit.
% We show the prevalence of infeasibilities and repeating solutions, and the significant effect of the early detection filters to avoid them. 
% In addition, %by reporting the results of the two phases separately, 
% we illustrate that 
Infeasibilities and repeating solutions are prevalent and the filters to avoid them give substantial benefit.
Phase II subsequently leads to fewer infeasibilities, which is one of our two main incentives ---the other being to focus on regions expected to yield desirable solutions.% (see %and the associated results are presented in
% Section~\ref{subsec:expresults_comparison}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Results from the regular version.}
% \label{subsubsec:expresults_2phase_regular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Table~\ref{tab:stats_regular} summarizes the results from {\twophasereg}. % for each phase and case. 
{\crevii The column labels are defined as follows:
\BI 
\I ``\# $\eps$-vectors" is the number of $\eps$-vectors constructed at the beginning of the phase (i.e., the cardinality of $\epsSetI$ or $\epsSetII$ in Figure~\ref{fig:flowchart}),
\I ``\# sol" is the number of obtained Pareto-optimal points,
\I ``\% sol" is the percentage of Pareto-optimal points with respect to the number of $\eps$-vectors,
\I ``\% infeas" is the percentage of $\eps$-vectors for which $\mopeps$ is infeasible,
\I ``\% omit in infeas" is the percentage of early-detected $\eps$-vectors among the infeasible cases,
\I ``\% omit for infeas" is the percentage of early-detected $\eps$-vectors for infeasibility (among all $\eps$-vectors),
\I ``\% omit for repeat" is the percentage of early-detected $\eps$-vectors for repeating solutions,
\I ``Unit sol time" is the average time to obtain a solution,
\I ``Total sol time" is the overall time spent solving all $\mopeps$ models.
\EI
}

\begin{comment}
{\crevii The column labels are ``\# $\eps$-vectors", ``\# sol", ``\% sol", ``\% infeas", ``\% omit in infeas", ``\% omit for infeas", ``\% omit for repeat", ``Unit sol time" and ``Total sol time".}
``\# $\eps$-vectors" denotes the number of $\eps$-vectors constructed at the beginning of the phase (i.e., the cardinality of $\epsSetI$ or $\epsSetII$ in Figure~\ref{fig:flowchart}), 
``\# sol" is the number of obtained Pareto-optimal points, 
and ``\% sol" is their percent ratio.  
Additionally, ``\% infeas" is the percentage of $\eps$-vectors for which $\mopeps$ is infeasible, and ``\% omit in infeas" denotes the percentage of $\eps$-vectors detected without solving the model. ``\% omit for infeas" 
% provides another statistic on the early infeasibility detection, namely 
is the percentage of $\eps$-vectors discarded early. % among all.
% ``\% omit in infeas" the percentage of $\eps$-vectors omitted among the infeasible, 
Similarly, ``\% omit for repeat" is the percentage of  $\eps$-vectors detected as repeating solutions. %discarded by early detection of repeating solutions.
Finally, ``Unit sol time" is the average time to obtain a solution, 
and ``Total sol time" is the overall time spent solving all $\mopeps$ models.
%, we report the number of inputted $\eps$-vectors (\# $\eps$-vectors), 
%the number of solutions obtained (\# sol), 
%the percentage of solutions obtained with respect to the number of $\eps$-vectors input (\% sol), 
% the percentage of $\eps$-vectors leading to infeasibility (\% infeas), 
% the percentage of $\eps$-vectors omitted for infeasibility (\% omit for infeas), 
% the percentage of $\eps$-vectors omitted among $\eps$-vectors leading to infeasibility (\% omit in infeas), 
% the percentage of $\eps$-vectors omitted to prevent repeating solutions (\% omit for repeat), 
% the average solution time to obtain one solution (Unit sol time), 
% and the total solution time (Total sol time).
% For each phase, the averages over all cases are also provided at the bottom row of each block.
\end{comment}


\input{Tables/table_stats_regular}

We observe that early detection of infeasibilities leaves a small proportion of $\eps$-vectors to be evaluated.
For Phase I, on average, 66.4\% of $\eps$-vectors are discarded for infeasibility, and only 0.9\% of the infeasible models are later considered. %, which makes 98.7\% of all infeasibilities being captured early. 
Together with an average 28.5\% of $\eps$-vectors discarded to eliminate repeating solutions, around 95\% of all $\eps$-vectors are omitted {\crevii in a negligible computation effort requiring around $10^{-4}$ seconds (thus not explicitly reported).}
%without being solved for, leading to a significant time saving, especially considering that the overall time spent for early detection is around $10^{-4}$ seconds only (thus not explicitly reported).
For Phase II, the average infeasibility percentage drops to 10.5\%, with more than half of those being detected early.
This shows that revision of objective ranges for Phase II concentrates the search as intended.  
The increased percentage of solutions in Phase II also indicates this fact, and the forthcoming Section~\ref{subsec:expresults_comparison} illustrates that the overall solution quality improves as planned.
Combined with the $\eps$-vectors omitted to avoid repeating solutions, an average of nearly 48\% of all $\eps$-vectors are discarded in Phase II, and we observe that the unit solution times are decreased. 
We note that, except for Cases 2 and 8, limits for tumor overdosing collapsed to zero, making $\numGrids^3$ $\eps$-vectors rather than $\numGrids^4$, with $\numGrids$ denoting the number of distinct $\eps_{\objIndex}$ values used for each objective, set to 10 and 5 for Phases I and II, respectively.


% In order to check the actual effect of the early detection of repeating solutions, we also tested {\twophasereg} without it.
We tested {\twophasereg} without the repeating solution filter to identify its impact.
Among the $\eps$-vectors that yield a solution in Phase I, only 0.34\% gives a solution not previously obtained but discarded with the early detection filter (due to existence of alternative optima).
%is active (due to existence of alternative optima), while 
We encountered no such solutions in Phase II.
Early detection eliminated around 93\% and 55\% of $\eps$-vectors that produced a solution in Phases I and II, with no repeating solutions, % that could not be detected.
% Among all the $\eps$-vectors that could yield a solution in Phase I, around 93\% is discarded, and only 0.34\% yields a solution not obtained before but is discarded (due to existence of alternative optima), while they are 55\% and none for Phase II, respectively.
so the early detection strategies significantly reduce calculations without jeopardizing Pareto representation.
% These results show that the early detection strategies spare a significant amount of time in general, with almost no loss of a distinct solution and inclusion of a repeating solution.
Run times of some cases (e.g., Case 4) may nevertheless be high due to the size and/or inherent difficulty of those instances.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Results from the ML-guided version.}
\label{subsubsec:expresults_2phase_ml}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\st{We first investigate the performance of the employed prediction models. As mentioned before, we trained random forest models for feasibility classifications first, and then for the prediction of coverage, PCI and BOT values. }
{\crevi % In order to decide on 
We selected the classification and regression models from several alternatives, %, as mentioned in Section~\ref{subsubsec:twophase_predictmodels}. 
% To this end, we took 
by taking the results from (the first round of) Phase I for each one of the eight cases, and using them as training data.
We performed a 5-fold cross validation 10 times for each model and case combination separately, and we compared the mean accuracy (proportion of correct classifications) and the area under the receiver operating characteristic curve for classifiers, and mean absolute error for regressors.
% and find that 
Random forests yielded the best overall performance with decision trees doing almost as well, probably because we only have four features (which is the length of an $\eps$-vector for our 5-objective model). For details, see Table~\ref{tab:ml_models_comparison} %\autoref{tab:ml_models_comparison} 
in Section~\ref{app:results} %\autoref{app:results} 
of the Online Supplement. }

{\crevi 
%\st{As mentioned before, we trained random forest models for feasibility classifications first, and then for the prediction of coverage, PCI and BOT values. We find that random forest models are performing very well. More specifically, }
We find upon comparing predictions with actual results that} feasibility classification is at least 96\% accurate on the average, and that mean absolute errors for Cov and PCI are approximately no greater than 2\%.
BOT values vary on a larger scale, which occasionally lead to relatively higher prediction errors.
Nevertheless, with a mean absolute error of less than seven (minutes), prediction performance for BOT remains useful. % useful and acceptable.
We note that it is possible to hedge against prediction inaccuracies by slightly relaxing the filtering threshold values, % used for filtering.
% For further details, 
see Table~\ref{tab:prediction_scores}  %\autoref{tab:prediction_scores} 
in Section~\ref{app:results} % \autoref{app:results} 
of the Online Supplement.


% Next, we evaluate the efficacy of {\twophaseml}.
% Overall, 
{\twophaseml} decreases the run times by nearly half.
%, compared to {\twophasereg}.
Specifically, in Phase I, with 8.6\% of the initially constructed $\eps$-vectors for {\twophasereg} on the average, {\twophaseml} 
%spends {\crevi 23\% to 72\% less time (for Case 1 only, {\twophaseml} spends a little more time)},
%\st{19\% to 62\% less time across the eight cases}
% amounting to an 
averages a {\crevi 47.6\%}
%\st{45.2\%} 
time saving. 
The number of $\eps$-vectors selected for Phase II of {\twophaseml} is 14.5\% of those built for the same phase of the regular version, and the time savings range from {\crevi 24\% to 79\%, averaging 46.5\%},
%\st{16\% to 91\%, making 51.8\%}
% on the average.
% For detailed results analogous to those in Table~\ref{tab:stats_regular}, 
see Table~\ref{tab:stats_ml} % \autoref{tab:stats_ml} 
in Section~\ref{app:results} %\autoref{app:results} 
of the Online Supplement.


% Having observed that the prediction models yield satisfactory performance, we next investigate the efficacy of {\twophaseml}. Table~\ref{tab:stats_ml} contains results analogous to those in Table~\ref{tab:stats_regular}. Here, we additionally report the percentage of $\eps$-vectors and run times relative to those from {\twophasereg}, under ``\% {\twophasereg} $\eps$-vectors" and ``\% {\twophasereg} time" headings, to reveal how much effort is saved via ML tools. Note that for Phase I, we give the number of $\eps$-vectors as an explicit sum of those used in two rounds, i.e., the size of the random sample of $\eps$-vectors from the first round plus the number of those found promising for the second round.

% In Phase I, with 8.6\% of $\eps$-vectors of {\twophasereg} on the average, 45.2\% overall run time reduction is achieved. For Case 4 in particular, which has the highest unit solution time, 2.4 hours of run time is saved in Phase I. Even though the objective ranges explored in Phase II mostly lead to desirable solutions, {\twophaseml} still achieves 51.8\% time saving in total. We note that Phase II time of Case 1 is indeed only 13.5 seconds more than that spent in {\twophasereg}, and this is simply due to random fluctuations in run times.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Solution Quality Assessment}
\label{subsec:expresults_comparison}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% After assessing the efficacy and efficiency of the proposed approach in the previous sections, 
% Lastly, we focus on the quality of the obtained solutions on the basis of clinical criteria.
% First, we present a summary of results in
Table~\ref{tab:comparison} contains summary statistics for Cov, PCI, BOT, and maximum OAR dose values of the two different versions of {\twophase} compared with those of {\cevikModel} and the clinical outcomes.
%, under three groups of columns for each one of the eight real cases.
% The first group is dedicated to {\twophase} and contains two rows for each case, the top one for {\twophasereg} (R), and the bottom for {\twophaseml} (ML).
% Because 
Our solution approach generates a collection of solutions for each case, and we report the number of Pareto-optimal 
% (with respect to the five MOLP objectives) 
points obtained and the number that remained after filtering dominated Cov, PCI, and BOT values (in parentheses next to the total number of solutions).
For Cov, PCI and BOT values, we report the minimums and maximums obtained. %, as well as the average and standard deviation values in a second line below (avg $\pm$ std).
% For cases that incorporate OARs (all such cases in our test bed have two OARs), 
We also list the average maximum dose each OAR received over the efficient solutions.



We see from Table~\ref{tab:comparison} that the maximum Cov and PCI, and the minimum BOT values are always better than the point values achieved clinically and by {\cevikModel}.
Comparing the performances of {\twophasereg} and {\twophaseml}, we observe that the latter yields average and minimum Cov and PCI values at least as good as those of the former. 
% and the maximum values are almost always the same, 
This is because {\twophaseml} has an extra filtering step to only generate desirable solutions in the second round of Phase I,  
% because it is designed to preferentially generate desirable solutions and avoid others as much as possible.
as a consequence of which it also yields fewer solutions than {\twophasereg}.
% However, the differences become smaller when we consider the number of solutions whose coverage, PCI and BOT values are not dominated by others (shown in parentheses).
% Also, 
{\crevii The minimum and maximum BOT values from {\twophasereg} and {\twophaseml} are almost identical --- the maximum BOT value allowed was three hours, as also reported in \citep{maxBOTref}.}
% the same, because BOT filtering is done only in Phase II for both. %versions. 
% We note that the maximum BOT value we allow in our experiments is three hours (even if the payoff table gives a larger value), since {\srs} treatment times vary up to that value \citep{maxBOTref}.


\input{Tables/table_comparison}

We next investigate the distribution of Pareto solutions
% individual solutions 
over the space of the three performance criteria in Figure~\ref{fig:cases1to4}.
For brevity we consider Cases 1 to 4 as representatives to show the different ways solutions are dispersed. % and present them here, while providing the 
Results for the remaining cases are provided in % in Figure~\ref{fig:cases5to8} in Section~\ref{app:results} %\autoref{app:results} 
the Online Supplement. 
Each row of Figure~\ref{fig:cases1to4} is dedicated to one case and contains two plots.
The plot on the left shows Cov versus PCI and the plot on the right displays BOT versus PCI for solutions yielding at least 99.7\% Cov.
This limit is higher than the maximum coverage achieved clinically and by {\cevikModel} over all eight cases, guaranteeing that our results on the right-hand side plots outperform clinical outcomes and {\cevikModel} results. % the others coverage-wise.
% The (teal blue) circular markers show the outputs from Phase I, and the (pink) triangular markers are from Phase II, with the filled markers being used for the outputs of {\twophaseml}. The (black) square and star markers represent the {\cevikModel} and clinical results, respectively. 

\input{Figures/fig_plots_cases1to4}

% We observe from 
Figure~\ref{fig:cases1to4} illustrates that the two phases of {\twophase} work as intended. 
While the solutions from Phase I are relatively scattered throughout the space of the three performance criteria, those from Phase II are typically clustered around more desirable regions.
The left-hand side plots demonstrate that {\twophasereg} is able to produce a considerably large collection of solutions outperforming the others in terms of both Cov and PCI, and {\twophaseml} identifies many such solutions.
% and a significant amount of such solutions can be captured by {\twophaseml}. 
% As for the plots on 
The right-hand side plots show that several of our solutions are significantly better than those from the clinical design or from {\cevikModel}.
% the others in all three aspects, except for Cases 2 and 4 out of eight.
Cases 2 and 4 are exceptions.
% For Case 2, 
A Cov of only 82\% has been achieved previously for Case 2, potentially due to clinicians' preference to keep the dose to OAR1 much lower than the predefined OAR1 dose limit (9.7 Gy vs 15.0 Gy). 
Our approach, however, produces solutions attaining essentially full coverage with higher, yet still realizable, BOT values, and hence, we provide the clinician options. %, in an automated manner, a wide range of possible treatment plans.
Moreover, we obtain many solutions with strictly better Cov, PCI, and BOT values than the others, which are not contained in the right-hand side plot because points with less than 99.7\% Cov are not shown.
% For Case 4, 
Almost all solutions for Case 4
% represented on the right-hand side plot 
are better than the others in terms of Cov and PCI, yet they yield relatively higher BOT values than that of {\cevikModel}.
The general distribution of solutions from Cases 5 to 8 are similar to that of Case 3, and thus our conclusions remain valid for them. 


{\crevi
We lastly examine the dose-volume histograms (DVHs) and isodose curves for a representative case, Case 3, see Figure~\ref{fig:DVH_isodose}. 
A DVH displays the fraction of each structure's volume receiving at least a certain amount of dose. We plot the relative dose percentages on the $x$-axis by proportioning the received doses to the prescription dose for the tumor and the maximum allowed doses for OARs. %, rather than absolute dose values (in units of Gy), 
Among the set of solutions obtained from {\twophasereg}, {\crevii we first remove solutions whose Cov is less than 99.7\% and whose PCI is less than 0.75.
We then discard solutions dominated in terms of the Cov, PCI and BOT.}
%we first filter the ones that yield at least 99.7\% coverage and 0.75 PCI value, then discard the ones that are dominated by some other solution in terms of the coverage, PCI, and BOT values. 
We plot the DVH curves for the remaining solutions that provide virtually full coverage, PCI values between 0.87 and 0.96, and BOT from 31 to 115 minutes.
% We then arbitrarily select one of these solutions  
{\crevii We then select a solution with 0.96 PCI and 101-minute BOT}
and plot the associated isodose curves for several cross sections of the tumor and OAR tissues.
For each cross section, we contour the areas that receive at least 50\% and 100\% of the prescribed dose for the tumor (12.5~Gy for Case~3), and indicate the tumor and nearby OAR tissues with shaded areas.
}

\input{Figures/fig_DVH_isodose}
%
{\crevi A DVH curve for the tumor should ideally mimic a vertical decay at the prescription dose, and in our case it is deviating only slightly from the reference line (shown with the gray vertical line).
% especially considering the maximum dose for the tumor is specified as twice the prescription dose in our cases, corresponding to 200\% relative dose.
Due to the proximity of the tumor to the brainstem and cochlea, which is evident from the cross sections depicted in the first three rows of the plots on the right in Figure~\ref{fig:DVH_isodose}, the 50\% isodose curves for the target intersect these organs. 
As the intersecting volume percentage of the cochlea is larger, we observe that its DVH curve starts decaying later than that of the brainstem.
However, the clinically prioritized measure for OARs is the maximum doses they receive, and they are less than 85--90\% of the allowed values.
%We observe from these plots that {\twophase} generates highly conformal treatment plans.
%Quote: To assess treatment quality, dose-volume histograms (DVHs) are employed. This histogram is a measure of the cumulative dose received by a given structure, specifying the fraction of each structure’s volume that receives at least a certain amount of dose. The DVH plots for healthy organs should fall as close to the origin as possible, while the DVH plot for the target structure should mimic a vertical line at the prescription dose.
}

\begin{comment}
\subsection{\cred Key Observations and Insights}
\label{subsec:expresults_discussion}

{\cblue When the sample size in the first round of Phase I is too small, it might be possible not to get any desirable solution. In such cases, one can take an additional sample of runs with the hope of capturing some samples as desired, or if it is not an option, the filtering criteria of predictions can be adjusted accordingly... .....}
\end{comment}

